Inference Attacks for X-Vector Speaker Anonymization

We revisit the privacy-utility tradeoff of x-vector speaker anonymization. Existing approaches quantify privacy through training complex speaker verification or identification models that are later used as attacks. Instead, we propose a novel inference attack for de-anonymization. Our attack is simple and ML-free yet we show experimentally that it outperforms existing approaches.

==> acknowledgements.tex <==
\section{Acknowledgements}

We thank the anonymous reviewers for their helpful comments on earlier versions of the paper. This work was supported in part by the National Science Foundation under CNS-2055123. Any opinions, findings, conclusions, or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of the National Science Foundation.
